Prediction of defect properties in concentrated solid solutions using a Langmuir-like model

The alleged existence of sluggish diffusion in high entropy alloys has drawn controversy. In high entropy alloys, and in general in all solids, transport properties are controlled by point defect concentration, which must be known before performing atomistic simulations to compute transport coefficients. In this work, we present a general Langmuir-like model for defect concentration in an arbitrarily complex solid solution and apply this model to generate expressions for concentrations of vacancies and small interstitial atoms. We then calculate the vacancy concentration as a function of temperature in the equiatomic CoNiCrFeMn and FeAl alloys with modified embedded-atom-method potentials for various chemical orderings, showing there is no clear correlation between vacancy thermodynamics and chemical ordering in the CoNiCrFeMn alloy but clear systematic patterns for FeAl. We believe this is due to the high stability of disordered, random and ordered, intermetallic phases respectively in the CoNiCrFeMn and FeAl systems. This work provides future avenues to the prediction of thermal interstitials and vacancies in solid solutions, which is necessary for models of non-equilibrium behavior of solid solutions.

==> sections/limits.tex <==
\section{Limits}

For substitutional impurities (atomic and vacancy), from Eq. \eqref{eq:local-prob}:

\begin{equation}
    \begin{aligned}
        \frac{1}{\sum_\alpha e^{\beta\mathcal{H}_\sigma^{(\alpha)}}} &= \frac{\pi_\sigma(\beta)}{1 - \pi_\sigma(\beta)}\\
        &= \pi_\sigma(\beta) + \mathcal{O}\left(\left[\pi_\sigma(\beta)\right]^2\right)
    \end{aligned}
\end{equation}

So, in the dilute limit, i.e. small $\pi_\sigma(\beta)$, the expressions for substitutional impurities (atomic and vacancy) are reduced to:

\begin{equation}\label{eq:small-sub}
    \pi_\sigma(\beta) \approx \frac{1}{\sum_\alpha e^{\beta\mathcal{H}_\sigma^{(\alpha)}}}
\end{equation}

and the expression for small impurities can be rewritten as:

\begin{equation}\label{eq:small-int}
    \pi_\sigma^{(\iota)}(\beta) = \frac{1}{\sum_\gamma e^{\beta \mathcal{H}_\sigma^{(\gamma)}}}
\end{equation}

where $\gamma\in\{\iota\}\cup\{(\iota, \iota')\;|\;\iota'\in\mathcal{I}\}$. Note that \eqref{eq:small-sub} and \eqref{eq:small-int} are only different in the sequence over which a summation is performed. Therefore, we can sum over $\mathcal{A}$ without loss of generality.

\subsection{Homogeneous Limit}

For a homogeneous medium with one possible impurity type, we have a unique enthalpic penalty $\mathcal{H} = \mathcal{H}_\sigma^{(\alpha)}$, so $\pi_\sigma(\beta) = x_\iota(\beta)$ for all sites $\sigma$. Therefore:

\begin{equation}
    x_\iota(\beta) = \frac{1}{e^{\beta\mathcal{H}}} = e^{-\beta\mathcal{H}}
\end{equation}

recovering the standard Arrhenius expression for impurity concentration.

\subsection{High Temperature Limit}

In the dilute limit:

\begin{equation}
    \ln \pi_\sigma(\beta) = -\ln\left(\sum_\alpha e^{\beta\mathcal{H}_\sigma^{(\alpha)}}\right)
\end{equation}

Defining a random variable $\mathcal{H}_\sigma^{(\mathcal{A})}$ by a uniform distribution over $\{\mathcal{H}_\sigma^{(\alpha)}\;|\; \alpha\in\mathcal{A}\}$ yields:

\begin{equation}
    \begin{aligned}
        \ln \pi_\sigma(\beta)
        &=\ln\frac{1}{|\mathcal{A}|} - \ln \mathbb{E}\left[ e^{\beta\mathcal{H}_\sigma^{(\mathcal{A})}}\right]
    \end{aligned}
\end{equation}

Then $\ln \mathbb{E}\left[e^{\beta\mathcal{H}_\sigma^{(\mathcal{A})}}\right]$ is a cumulant generating function (CGF) of the random variable $\mathcal{H}_\sigma^{(\mathcal{A})}$ (assuming the random variable is temperature-independent), and can thus be expanded in powers of $\beta$ with cumulants $\kappa_\sigma^{(\ell)}$ as coefficients to some finite order $n$ \cite{brillinger_timeseries}:

\begin{equation}
    \pi_\sigma^{(n)}(\beta) = \frac{1}{|\mathcal{A}|}\exp\left( - \sum_{\ell=1}^n \frac{\kappa_\sigma^{(\ell)}}{\ell!}\beta^\ell\right)
\end{equation}

where $\pi_\sigma^{(n)}(\beta) \to \pi_\sigma(\beta)$. Then:

\begin{equation}
    x_\iota^{(n)}(\beta) = \frac{1}{|\mathcal{A}|} \left\langle\exp\left( - \sum_{\ell=1}^n \frac{\kappa_\sigma^{(\ell)}}{\ell!}\beta^\ell\right)\right\rangle
\end{equation}

where $x_\iota^{(n)}(\beta)\to x_\iota(\beta)$. Define the $n$-dimensional random variable $\mathbf{k}_\sigma$ as:

\begin{equation}
    \mathbf{k}_\sigma = -\left(\kappa_\sigma^{(1)}, \frac{\kappa_\sigma^{(2)}}{2}, \cdots, \frac{\kappa_\sigma^{(n)}}{n!}\right)
\end{equation}

and the variable $\mathbf{b}(\beta)$ as:

\begin{equation}
    \mathbf{b} = \left(\beta, \beta^2, \cdots, \beta^n\right)
\end{equation}

Therefore:

\begin{equation}
    \ln x_\iota^{(n)}(\beta) = \ln\frac{1}{|\mathcal{A}|} + \ln\left\langle e^{\mathbf{b}(\beta)\cdot \mathbf{k}_\sigma}\right\rangle
\end{equation}

where $\ln\left\langle e^{\mathbf{b}(\beta)\cdot\mathbf{k}_\sigma}\right\rangle$ is another CGF. Expanding this CGF about $\mathbf{b}(\beta) = \mathbf{0}$ gives:

\begin{equation}
    \begin{aligned}
        \ln x_\iota^{(n)}(\beta) &= \ln\frac{1}{|\mathcal{A}|} + \left\langle\mathbf{k}_\sigma\right\rangle\cdot \mathbf{b}(\beta)\\
        &+ \frac{1}{2}\mathbf{b}(\beta)\cdot\mathbf{K}\mathbf{b}(\beta) + \cdots
    \end{aligned}
\end{equation}

where $\mathbf{K}$ is the covariance matrix with elements $K_{\ell\ell'}$:

\begin{equation}
    K_{\ell\ell'} = \frac{1}{\ell!\ell'!}\left\langle \left(\kappa_\sigma^{(\ell)} - \left\langle\kappa_\sigma^{(\ell)}\right\rangle\right)\left(\kappa_\sigma^{(\ell')} - \left\langle \kappa_\sigma^{(\ell')}\right\rangle\right)\right\rangle
\end{equation}

Therefore:

\begin{equation}
    x_\iota^{(n)}(\beta) = \frac{1}{|\mathcal{A}|}e^{-\beta\left\langle\kappa_\sigma^{(1)}\right\rangle -\frac{1}{2}\beta^2\left(\left\langle\kappa_\sigma^{(2)}\right\rangle - K_{11}\right) + \mathcal{O}\left(\beta^3\right)}
\end{equation}

So, in the high-temperature limit, we recover an Arrhenius expression with activation energy $\left\langle\frac{1}{|\mathcal{A}|}\sum_\alpha\mathcal{H}_\sigma^{(\alpha)}\right\rangle$.
